Performance bottlenecks detection through microarchitectural sensitivity

Modern Out-of-Order (OoO) CPUs are complex systems with many components interleaved in non-trivial ways. Pinpointing performance bottlenecks and understanding the underlying causes of program performance issues are critical tasks to make the most of hardware resources. We provide an in-depth overview of performance bottlenecks in recent OoO microarchitectures and describe the difficulties of detecting them. Techniques that measure resources utilization can offer a good understanding of a program's execution, but, due to the constraints inherent to Performance Monitoring Units (PMU) of CPUs, do not provide the relevant metrics for each use case. Another approach is to rely on a performance model to simulate the CPU behavior. Such a model makes it possible to implement any new microarchitecture-related metric. Within this framework, we advocate for implementing modeled resources as parameters that can be varied at will to reveal performance bottlenecks. This allows a generalization of bottleneck analysis that we call sensitivity analysis. We present Gus, a novel performance analysis tool that combines the advantages of sensitivity analysis and dynamic binary instrumentation within a resource-centric CPU model. We evaluate the impact of sensitivity on bottleneck analysis over a set of high-performance computing kernels.

==> src/harness.tex <==
\begin{figure*}
    \definecolor{col_bench_gen}{HTML}{5a7eff}
    \definecolor{col_bench_gen_bg}{HTML}{dbeeff}
    \definecolor{col_bench_harness}{HTML}{ffa673}
    \definecolor{col_results}{HTML}{000000}
\centerline{
  \begin{tikzpicture}[
      hiddennode/.style={rectangle,draw=white, very thick, minimum size=5mm, align=center, font=\footnotesize},
      normnode/.style={rectangle,draw=black, very thick, minimum size=5mm, align=center, font=\footnotesize},
  resultnode/.style={rectangle,draw=col_results, fill=black!2, very thick, minimum size=5mm, align=center, font=\footnotesize},
  bluenode/.style={rectangle, draw=col_bench_gen, fill=col_bench_gen_bg, very thick, minimum height=5mm, minimum width=4cm, align=center, font=\footnotesize},
  rednode/.style={rectangle, draw=col_bench_harness, fill=orange!5, very thick, minimum size=5mm, align=center, font=\footnotesize},
  bencher/.style={rednode, minimum width=2.5cm, minimum height=5mm},
  genarrow/.style={draw=col_bench_gen},
  harnarrow/.style={draw=col_bench_harness},
  ]
  \centering
  %Nodes
  \node[bluenode]  (bench)                       {Benchmark suite};
  \node[bluenode]  (pocc)     [below=of bench] {Loop nest optimizers};
  \node[bluenode]  (kernel)   [below=of pocc]    {Microkernel extraction};
  \node[bluenode]  (gcc)      [below=of kernel]  {Compilations};
  \node[rednode]   (gdb)      [right=0.1\textwidth of gcc] {Basic block \\extraction};
  \node[bencher]   (ithemal)  [right=4cm of gdb]   {Ithemal};
  \node[bencher]   (iaca)     [above=0.5em of ithemal]    {IACA};
  \node[bencher]   (uica)     [above=0.5em of iaca]    {uiCA};
  \node[bencher]   (llvm)     [above=0.5em of uica]     {llvm-mca};
  \node[bencher]   (bhive)    [above=0.5em of llvm]     {BHive (measure)};
  \node[rednode]   (ppapi)    [left=1cm of bhive]   {perf (measure)};
  \node[rednode]   (gus)      [below=0.5em of ppapi] {Gus};
  %% \node[rednode]   (uica)     [below=of gdb]     {uiCA};
  \node[rednode]   (lifting)  [right=of bhive]   {
      Prediction lifting};
  \node[
    draw=black,
    very thick,
    dotted,
    fit=(ppapi) (gus) (bhive) (llvm) (uica) (iaca) (ithemal)
  ] (comps) {};
  \node (throughput_label)  [above=0.2em of comps,align=center] {
          \footnotesize Throughput predictions \\\footnotesize \& measures};
  \node[draw=black,
    very thick,
    dotted,
    %% label={below:\footnotesize Variations},
    label={[above,xshift=1.5cm]\footnotesize Transformations },
    fit=(pocc) (kernel) (gcc)
  ] (vars) {};
\node[resultnode]  (bench2) [below=of lifting] {Evaluation metrics \\ for
        code analyzers};

  % Key
  \node[]  (keyblue1)     [below left=0.7cm and 0cm of vars]   {};
  \node[hiddennode]  (keyblue2)     [right=0.5cm of keyblue1]   {Generating microbenchmarks};
  \node[]  (keyred1)     [right=0.6cm of keyblue2]   {};
  \node[hiddennode]  (keyred2)     [right=0.5cm of keyred1] {Benchmarking harness};
  \node[]  (keyresult1)     [right=0.6cm of keyred2]   {};
  \node[hiddennode]  (keyresult2)     [right=0.5cm of keyresult1]
      {Results analysis};

  %Lines
    \draw[-, very thick, harnarrow] (keyred1.east)     -- (keyred2.west);
    \draw[-, very thick, genarrow]  (keyblue1.east)     -- (keyblue2.west);
    \draw[-, very thick]  (keyresult1.east)     -- (keyresult2.west);
  \draw[->, very thick, genarrow]   (bench.south)   -- (pocc.north);
  \draw[->, very thick, genarrow]   (pocc.south)    -- (kernel.north);
  \draw[->, very thick, genarrow]   (kernel.south)  -- (gcc.north);
  \draw[->, very thick, genarrow]   (gcc.east)     -- (gdb.west);
  \draw[->, very thick, genarrow]   (gcc.east)     -- (ppapi.west);
  \draw[->, very thick, genarrow]   (gcc.east)     -- (gus.west);
  \draw[->, very thick, harnarrow]  (gdb.east)     -- (uica.west);
  \draw[->, very thick, harnarrow]  (gdb.east)     -- (iaca.west);
  \draw[->, very thick, harnarrow]  (gdb.east)     -- (ithemal.west);
  \draw[->, very thick, harnarrow]  (gdb.east)     -- (bhive.west);
  \draw[->, very thick, harnarrow]  (gdb.east)     -- (llvm.west);
  \draw[->, very thick, harnarrow]  (comps.east|-lifting)   -- (lifting.west);
  \draw[->, very thick]            (lifting.south)   -- (bench2.north);
  \end{tikzpicture}
}
\vspace{-1em}
\caption{Our analysis and measurement environment.\label{fig:contrib}}
\vspace{-1em}
\end{figure*}


==> src/rob_bottleneck.tex <==
\begin{figure}
  \footnotesize
  \begin{center}
    \begin{tabu}{ | c | c c c c c c c c | }
      \hline
      \muop{s} sequence & \micro{1} & \micro{2} & \micro{3} & \micro{4} & \micro{5} & \micro{6} & \micro{7} & \micro{8} \\ 
      \hline
      mapped ports      & p0 & p0  & p1 & p1  & p2 & p3 & p2  & p1  \\
      \hline
      timestamps        & 0  & 1   & 0  & 1   & 2  & 2  & 3   & 3   \\
      \hline \rowfont{\color{blue}}
      p0 accelerated    & 0  & 0.5 & 0  & 1   & 1  & 1  & 2   & 2   \\
      \hline \rowfont{\color{blue}}
      p1 accelerated    & 0  & 1   & 0  & 0.5 & 2  & 2  & 3   & 3   \\
      \hline \rowfont{\color{blue}}
      p2 accelerated    & 0  & 1   & 0  & 1   & 2  & 2  & 2.5 & 2.5 \\
      \hline \rowfont{\color{blue}}
      p3 accelerated    & 0  & 1   & 0  & 1   & 2  & 2  & 3   & 3   \\
      \hline
    \end{tabu} \\
    \vspace{0.3cm}
    $ROB_0$:
    \begin{tabular}{ | c | }
      \hline 
      \micro{3}(p1) \\
      \micro{2}(p0) \\
      \micro{1}(p0) \\
      \hline 
    \end{tabular}
    \hspace{0.3cm}
    \begin{tabular}{ | c | }
      \hline 
      \textcolor{gray}{\micro{3}(p1)} \\
      \micro{2}(p0) \\
      \textcolor{gray}{\micro{1}(p0)} \\
      \hline 
    \end{tabular}
    \hspace{0.3cm}
    $ROB_1$:
    \begin{tabular}{ | c | }
      \hline
      \micro{4}(p1) \\
      \textcolor{gray}{\micro{3}(p1)} \\
      \micro{2}(p0) \\
      \hline 
    \end{tabular}
    \hspace{0.3cm}
    \begin{tabular}{ | c | }
      \hline
      \textcolor{gray}{\micro{4}(p1)} \\
      \textcolor{gray}{\micro{3}(p1)} \\
      \textcolor{gray}{\micro{2}(p0)} \\
      \hline 
    \end{tabular} \\
    \vspace{0.3cm}
    $ROB_2$:
    \begin{tabular}{ | c | }
      \hline 
      \micro{7}(p2) \\
      \micro{6}(p3) \\
      \micro{5}(p2) \\
      \hline 
    \end{tabular}
    \hspace{0.3cm}
    \begin{tabular}{ | c | }
      \hline 
      \micro{7}(p2) \\
      \textcolor{gray}{\micro{6}(p3)} \\
      \textcolor{gray}{\micro{5}(p2)} \\
      \hline 
    \end{tabular}
    \hspace{0.3cm}
    $ROB_3$:
    \begin{tabular}{ | c | }
      \hline
      \\
      \micro{8}(p1) \\
      \micro{7}(p2) \\
      \hline 
    \end{tabular}
    \hspace{0.3cm}
    \begin{tabular}{ | c | }
      \hline
      \\
      \textcolor{gray}{\micro{8}(p1)} \\
      \textcolor{gray}{\micro{7}(p2)} \\
      \hline 
    \end{tabular}
  \end{center}
  \caption{The simulated execution of a 8-\muop{s} program
    with no memory or register dependencies and with a ROB of
    size 3. The evolution of the latter over time is shown below
    ($ROB_t$ describes the state of the ROB at the time $t$).
    The black rows of the table above give an overview of the cycle stalling
    mechanism, with 1- the \muop{s} sequence, 2-the mapped port of each
    \muop{} and 3- the date on which each of them is executed assuming that
    each port has a throughput of 1 \muop{} per cycle.
    The blue rows simulate program execution by sensitivity,
    successively accelerating each of the 4 ports.
  \label{fig:rob_bottleneck}}
\end{figure}

